A General Framework for Analyzing Stochastic Dynamics in Learning Algorithms

One of the challenges in analyzing learning algorithms is the circular entanglement between the objective value and the stochastic noise. This is also known as the "chicken and egg" phenomenon and traditionally, there is no principled way to tackle this issue. People solve the problem by utilizing the special structure of the dynamic, and hence the analysis would be difficult to generalize. In this work, we present a streamlined three-step recipe to tackle the "chicken and egg" problem and give a general framework for analyzing stochastic dynamics in learning algorithms. Our framework composes standard techniques from probability theory, such as stopping time and martingale concentration. We demonstrate the power and flexibility of our framework by giving a unifying analysis for three very different learning problems with the last iterate and the strong uniform high probability convergence guarantee. The problems are stochastic gradient descent for strongly convex functions, streaming principal component analysis, and linear bandit with stochastic gradient descent updates. We either improve or match the state-of-the-art bounds on all three dynamics.

==> app-SGD.tex <==

Let $F$ be a convex function over some convex domain $\cW$ equipped with norm $\|\cdot\|$. For $G > 0$, a $G$-bounded stochastic gradient oracle on input $\bw$ returns a random $\hat{\bg}$, such that $\Exp[\hat{\bg}]$ is the subgradient of $F$ at $\bw$ and $\|\hat{\bg}\|\leq G$ almost surely. The SGD algorithm minimizes $F$ over $\cW$ with the help of this stochastic gradient oracle, maintaining a vector $\bw_t$ at time $t$ as follows.

\vspace{0.5cm}
\begin{algorithm}[H] 
	\caption{SGD for strongly convex function}\label{alg:SGD for strongly convex}
	    \textbf{Input:} Time parameter $T\in\N$ and step size parameters $\{\eta_t\}_{t\in\N}$.\\
	    \textbf{Initialize:} $\bw_0\in\cW$.\\
	    \For{$t=1,\dots,T$}{
	    Query the stochastic gradient oracle of $F$ at $\bw_{t-1}$ and get $\hat{\bg}_t$.\\
	    Let $\bw_t=\textsf{Proj}_{\cW}(\bw_{t-1}-\eta_t\hat{\bg}_t)$ where $\textsf{Proj}_{\cW}$ is an orthogonal projection operator for $\cW$.}
	    \textbf{Output:} $\bw_T$.
\end{algorithm}
\vspace{0.5cm}

We say $F$ is $\lambda$-strongly convex for some $\lambda>0$ if for all $\bw,\bw'\in\cW$ and any subgradient $\bg$ at $\bw$,
\[
F(\bw')\geq F(\bw)+\bg^\top(\bw'-\bw)+\frac{\lambda}{2}\|\bw'-\bw\|^2 \, .
\]
Due to strong convexity, there exists a unique minimizer $\bw^*\in\cW$ of $F$. Thus, the potential function is defined as $X_t=\|\bw_t-\bw^*\|^2$. Note again, due to strong convexity, 
\[
G\|\bw - \bw^*\|\geq \|\bg\|\cdot\|\bw - \bw^*\|\geq \langle \bg, \bw - \bw^* \rangle\geq \frac{\lambda}{2}\|\bw - \bw^*\|^2\, ,
\]
where $\bg$ is the gradient of $\bw$. This immediately yields that,
\[
\ X_t\leq \frac{4G^2}{\lambda^2}\, ,
\]
almost surely. The goal is to prove the following theorem, which is a formal version of~\autoref{thm:sgd}.

\begin{theorem}[Convergence of SGD for strongly convex functions]\label{thm: sgd main appendix}
Let $F$ be a $\lambda$-strongly convex function over some convex domain. An SGD algorithm with gradient bounded by $G>0$ almost surely has the following convergence rate. For every $\delta\in(0,1)$,
\begin{itemize}
\item if $\eta_t=1/(\lambda t)$, we have the following last iterate convergence
\[
\Pr\left[ X_{T} > \frac{1000G^2\log\frac{1}{\delta}}{\lambda^2T} \right] < \delta
\]
for every $T\in\N$;
\item if $\eta_t=1/(\lambda t)$, we have the following strong uniform convergence
\[
\Pr\left[\exists  t\in\N,\ X_{t} > \frac{1000 G^2\left(\log\frac{1}{\delta}+2\log\log(t+1)\right)}{\lambda^2 t} \right] < \delta \, ;
\]
\end{itemize}
\end{theorem}



\paragraph{Section structure.} In the rest of this section, we provide the recursion analysis in~\autoref{app:sgd recursion}, the moment and concentration analysis in~\autoref{app:sgd moment}, and the improvement analysis in~\autoref{app:sgd improvement}.

\subsection{Recursion analysis}\label{app:sgd recursion}
We linearize the process $X_t$. For every $0\leq T_0<T_1$, we rewrite $w_t$ using the update rule from \autoref{alg:SGD for strongly convex} and expand the term to yield,
\begin{align*}
X_t&=\|\bw_t-\bw^*\|^2=\|\textsf{Proj}_{\cW}(\bw_{t-1}-\eta_t\hat{\bg}_t)-\bw^*\|^2\leq \|\bw_{t-1}-\eta_t\hat{\bg}_t-\bw^*\|^2\\
%&=\|\bw_{t-1}-\bw^*\|^2-2\eta_t\hat{\bg}_t^\top(\bw_{t-1}-\bw^*)+\eta_t^2\|\hat{\bg}_t\|^2 \\
&=(1-2\eta_t\lambda)X_{t-1}+2\eta_t\left(\lambda X_{t-1}-\hat{\bg}_t^\top(\bw_{t-1}-\bw^*)\right)+\eta_t^2\|\hat{\bg}_t\|^2 \, .
\end{align*}

Let $M_{t}=\sum_{t'=T_0+1}^t\frac{2\eta_{t'}\left(\lambda X_{t'-1}-\hat{\bg}_{t'}^\top(\bw_{t'-1}-\bw^*)\right)+\eta_{t'}^2\|\hat{\bg}_{t'}\|^2}{\prod_{t''=T_0+1}^{t'}(1-2\eta_{t''}\lambda)}$ for all $T_0+1\leq t\leq T_1$. We unfold the recursion and obtain the following,
\[
X_t = \prod_{t'=T_0+1}^t(1-2\eta_{t'}\lambda)\left(X_{T_0} + M_{t}\right) \, .
\]

\subsection{Moment and concentration analysis}\label{app:sgd moment}
Next, we calculate a moment profile for the recursion in~\autoref{app:sgd recursion}.

\begin{lemma}[Moment profile for SGD]\label{lem:sgd moment details}
Consider the setting in~\autoref{thm: sgd main appendix}. Let $\Lambda > 0$ \& $\tau$ be the stopping time of the event $\lbrace X_t > \Lambda \rbrace$. For every $T_0+1\leq t\leq T$, the following functions $(B_{T_0},\mu_{T_0},\sigma^2_{T_0})$ form a moment profile for $\{X_t\}$, $\Lambda$, and $T_0$.
\begin{itemize}[leftmargin=*]
\item (Bounded difference) $|M_{t\wedge\tau}-M_{(t-1)\wedge\tau}|\leq B(t,\Lambda)=\eta_{t}\cdot\frac{12G/\lambda+\eta_{t}G^2}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)}$ almost surely.
\item (Conditional expectation) $\Exp\left[M_{t\wedge\tau}-M_{(t-1)\wedge\tau}\ |\ \cF_{t-1}\right]\leq\mu(t,\Lambda)=\eta_{t}^2\cdot\frac{G^2}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)}$.
\item (Conditional variance) $\Var\left[M_{t\wedge\tau}-M_{(t-1)\wedge\tau} \ |\ \cF_{t-1}\right]\leq\sigma^2(t,\Lambda)=\eta_{t}^2\cdot\frac{72G^2\Lambda+2\eta_{t}^2G^4}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)^2}$.
\end{itemize}
Specifically, if $\eta_t=1/(\lambda t)$ and $T_0 \geq100$, we can pick
\[
B_{T_0}(t,\Lambda) =\frac{20G^2t}{\lambda^2 T_0^2} \, ,\mu_{T_0}(t,\Lambda)=\frac{2G^2}{\lambda^2T_0^2} \, \text{, and }
\sigma_{T_0}^2(t,\Lambda) = \frac{G^2t^2}{\lambda^2T_0^4}\left(80\Lambda+\frac{3G^2}{\lambda^2t^2}\right)  \, .
\]
\end{lemma}
\begin{proof}
For bounded difference, we have
\begin{align}
|M_{t\wedge\tau}-M_{(t-1)\wedge\tau}| &= \left| \mathbf{1}_{\tau\geq t} \frac{2\eta_t\left(\lambda X_{t-1}-\hat{\bg}_t^\top(\bw_{t-1}-\bw^*)\right)+\eta_t^2\|\hat{\bg}_t\|^2}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)} \right| \, . \label{eq: sgd moment diff}
\intertext{By the Cauchy-Schwarz inequality and the facts that $\|\hat{\bg}_{t}\|\leq G$ and $X_t \leq \frac{4G^2}{\lambda^2}$, we get}
&\leq \mathbf{1}_{\tau\geq t} \eta_{t}\cdot  \frac{2\lambda X_{t-1} + 2G\sqrt{X_{t-1}} + \eta_tG^2}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)} \,
\leq \eta_{t}\frac{12G^2/\lambda + \eta_tG^2}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)} \, . \label{eq: sgd bounded difference}
\end{align}

\noindent For conditional expectation, we apply the fact that $\Exp[\hat{\bg}_{t}^\top(\bw_{t-1}-\bw^*)\ |\ \cF_{t-1}]\geq\lambda X_{t-1}$ to \autoref{eq: sgd moment diff} and obtain,
\begin{align}\label{eq: sgd bound conditional expectation}
    \Exp\left[M_{t\wedge\tau}-M_{(t-1)\wedge\tau}\ |\ \cF_{t-1}\right]\leq\eta_{t}^2\cdot\frac{G^2}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)} \, .    
\end{align}

For the conditional variance, we have by~\autoref{eq: sgd bounded difference} and the definition of $\tau$,
\begin{align}\label{eq: sgd bound conditional variance}
    \Var\left[M_{t\wedge\tau}-M_{(t-1)\wedge\tau} \ |\ \cF_{t-1}\right]\leq \Exp\left[\mathbf{1}_{\tau \geq t}\cdot(M_t-M_{t-1})^2\ |\ \cF_{t-1}\right]\leq \eta_{t}^2\cdot\frac{72G^2\Lambda+2\eta_{t}^2G^4}{\prod_{t'=T_0+1}^{t}(1-2\eta_{t'}\lambda)^2} \, .    
\end{align}

Notice that for $t>T_0\geq 100$
\begin{equation}\label{eq: sgd learning rate product}
\prod_{t' = T_0 + 1}^{t} (1 - 2\eta_{t'}\lambda) = \frac{T_0(T_0-1)}{t(t-1)}\geq \frac{99T_0^2}{100t^2} \, .   
\end{equation}

Plugging $\eta_t = \frac{1}{\lambda t}$ back into \autoref{eq: sgd bounded difference}, \autoref{eq: sgd bound conditional expectation} and \autoref{eq: sgd bound conditional variance} yields the final bounds.
\end{proof}


\subsection{Improvement analysis}\label{app:sgd improvement}

\subsubsection{Last iterate convergence}

\begin{proof}[Proof of item 1 of~\autoref{thm: sgd main appendix}]

In the analysis for last iterate convergence we consider a different stopping time $\tau$ defined for the event $\{X_t>\Lambda_t\}$, where $\Lambda_t = \frac{T_1}{t^2}\Lambda$, for an appropriate $\Lambda$ chosen later. Let $T_0=100$ and let $(B_{T_0},\mu_{T_0},\sigma^2_{T_0})$ be the moment profile obtained from~\autoref{lem:sgd moment details}. By concentration implied by \autoref{lem:martingale concentration}, we have
\[
\Pr\left[\exists T_0+1\leq t\leq T_1,\ |M_{t\wedge\tau}|>\Delta\right]<\delta\, ,
\]
where
\[
\Delta=2\max\left\{\sqrt{\sum_{t=T_0+1}^{T_1}\sigma^2_{T_0}(t,\Lambda_t)\log\frac{1}{\delta}},\ \max_{T_0+1\leq t\leq T_1}B_{T_0}(t,\Lambda_t)\log\frac{1}{\delta}\right\}+\sum_{t=T_0+1}^{T_1}\mu_{T_0}(t,\Lambda_t) \, .
\]
The deviation $\Delta$ can hence be written out as follows.
\begin{align*}
\Delta&\leq2\max\left\{\sqrt{\sum_{t=T_0+1}^{T_1}\frac{G^2t^2(80T_1\Lambda/t^2+3G^2/(\lambda^2t^2))}{\lambda^2T_0^4}\log\frac{1}{\delta}},\ \max_{T_0+1\leq t\leq T_1}\frac{20G^2t}{\lambda^2T_0^2}\log\frac{1}{\delta}\right\}+\sum_{t=T_0+1}^{T_1}\frac{2G^2}{\lambda^2T_0^2}\\
&%\leq2\max\left\{\frac{100G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2}\sqrt{\frac{\lambda^2\Lambda}{125G^2\log\frac{1}{\delta}}+\frac{1}{10T_1\log\frac{1}{\delta}}},\ \frac{20G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2}\right\}+\frac{2G^2T_1}{\lambda^2T_0^2} \, .
\leq2\max\left\{\frac{G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2}\sqrt{\frac{80\lambda^2\Lambda}{G^2\log\frac{1}{\delta}}+\frac{3}{T_1\log\frac{1}{\delta}}},\ \frac{20G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2}\right\}+\frac{2G^2T_1}{\lambda^2T_0^2} \, .
%\intertext{Letting $\Lambda=\frac{10000G^2\log\frac{1}{\delta}}{\lambda^2}$, we further have}
\intertext{Letting $\Lambda=\frac{G^2\log\frac{1}{\delta}}{\lambda^2}$, we further have}
%&\leq\frac{900G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2} \, .
&\leq\frac{42G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2} \, .
\end{align*}
\Jnote{Can somebody please verify my calculation above once? I have left the original calculation in comments in case I have made a mistake. I think this is tight (in the sense of having whole numbers). The below still needs to be modified.}

Now, in order to \textit{pull out} the stopping time $\tau$, we verify the pull-out condition stated in~\autoref{lem:pull out}, which is that,
\[
\Pr[\tau\geq t+1\, |\, M_{t'}\leq\Delta,\ \forall t'\leq t]=1\, ,
\]
for every $T_0+1\leq t\leq T_1$. Observe that when $M_{t'}\leq\Delta$ for all $t'\leq t$, for every $T_0+1\leq t'\leq t$, by the recursion we have 
\begin{align*}
X_{t'}&=\prod_{t''=T_0+1}^{t'}(1-2\eta_{t''}\lambda)(X_{T_0}+M_{t'}) =\frac{T_0(T_0-1)}{t'(t'-1)}(X_{T_0}+M_{t'})\\
&\leq\frac{T_0^2}{t'^2}(X_{T_0}+\Delta) \leq\frac{T_0^2}{t'^2}\frac{2000G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2}\\
&\leq\frac{T_1\Lambda}{10t'^2}=\frac{\Lambda_{t'}}{10}
\end{align*}
and hence $\tau>t'$ by the definition of $\tau$. Since the above holds for all $T_0+1\leq t'\leq t$, we have $\tau\geq t+1$ as desired. Finally, by the pull-out lemma (i.e.,~\autoref{lem:pull out}) we have
\[
\Pr\left[\exists T_0+1\leq t\leq T_1,\ |M_{t}|>\frac{900G^2T_1\log\frac{1}{\delta}}{\lambda^2T_0^2}\right]<\delta \, .
\]
Combine with the recursion and the fact that $X_{T_0}\leq\frac{4G^2}{\lambda^2}$ due to the $G$-boundedness of $F$, we have
\[
\Pr\left[X_{T_1}>\frac{1000G^2\log\frac{1}{\delta}}{\lambda^2T_1}\right]<\delta \, .
\]
This completes the proof for the last iterate convergence of SGD.
\end{proof}


\subsubsection{Strong uniform convergence}\label{app:sgd strong unif}
Recall that in~\autoref{sec:sgd} we used an interval analysis to achieve a tighter improvement analysis for the strong uniform guarantee. Here, we modularize the improvement analysis for a single interval into the lemma.

\begin{lemma}\label{lem:sgd concentration details}
Consider the setting in~\autoref{thm: sgd main appendix}. For every $100\leq T_0\in\N$, let  $(B_{T_0},\mu_{T_0},\sigma^2_{T_0})$ be the moment profile for $\{X_t\}$ and $T_0$ from~\autoref{lem:sgd moment details}. If $\eta_t=1/\lambda t$, then for every $A_0>A_1>0$, $\delta'>0$, $\Lambda>0$, and $100\leq T_0<T_1\in\N$, let
\[
\Delta=\frac{G^2T_1\log\frac{1}{\delta'}}{\lambda^2T_0^2} \left(\sqrt{\frac{70T_1\Lambda\lambda^2}{G^2
\log\frac{1}{\delta'}}} + 50\right) \, .
\]
Suppose that we have $A_0 + \Delta < \Lambda$ and $\frac{T_0(T_0-1)}{T_1(T_1-1)} \Lambda < A_1$. Then, 
\[
\Pr\left[\exists{T_0 + 1\leq t\leq T_1}\, ,\ X_t > \frac{T_0(T_0-1)}{t(t-1)}\cdot\Lambda \ \middle| \ X_{T_0} < A_0\right] < \delta' \, .
\]
In particular, the above implies $\Pr[X_{T_1}>A_1\ |\ X_{T_0}\leq A_0]\leq\delta'$.
\end{lemma}
\begin{proof}
Given the moment profile for $\{X_t\}$ in~\autoref{lem:sgd moment details}, we apply~\autoref{prop:concentration} and get the following deviation using~\autoref{lem:martingale concentration}.
\begin{align*}
 &2\max\left\lbrace\sqrt{\sum_{t' = T_0 + 1}^{T_1}\sigma_{T_0}^2(t', \Lambda)\log\frac{1}{\delta'}}, 2\max_{T_0+1\leq t'\leq T_1}B_{T_0}(t',\Lambda)\log\frac{1}{\delta'}\right\rbrace + \sum_{t'=T_0+1}^{T_1}\mu_{T_0}(t', \Lambda)\\
 =\ &\max\left\{2\sqrt{\sum_{t' = T_0 + 1}^{T_1}\frac{G^2t'^2}{\lambda^2T_0^4}\left(80\Lambda+\frac{3G^2}{\lambda^2t'^2}\right)\log\frac{1}{\delta'}} , 40\frac{G^2T_1}{\lambda^2T_0^2}\log\frac{1}{\delta'}\right\} + \sum_{t'=T_0+1}^{T_1}\frac{2G^2}{\lambda^2 T_0^2}\\
 \leq\ & \sqrt{\frac{70G^2T_1^3\Lambda\log\frac{1}{\delta'}}{\lambda^2T_0^4}} + \frac{G^2\sqrt{12\log\frac{1}{\delta'}}}{\lambda^2T_0^2} +  40\frac{G^2T_1}{\lambda^2T_0^2}\log\frac{1}{\delta'} + \frac{2G^2T_1}{\lambda^2 T_0^2}\\
 \leq\ &\frac{G^2T_1\log\frac{1}{\delta'}}{\lambda^2T_0^2} \left(\sqrt{\frac{70T_1\Lambda\lambda^2}{G^2
\log\frac{1}{\delta'}}} + 50\right) = \Delta \, .
\end{align*}
Next, by~\autoref{prop:concentration} we get the desiring improvement inequalities.
\end{proof}

We now prove the \textit{strong uniform} convergence bound.
\begin{proof}[Proof of item 2 in~\autoref{thm: sgd main appendix}]
Let $\ell=\infty$ and let
\[
t_0 = 0,\ t_1 = 100,\ t_i = 2t_{i-1},\ \forall i\geq2 \, .
\]
For $i\geq 1$, let
\[
\delta_i=\frac{\delta}{2i^2},\ a_0 = \frac{1000 G^2\log\frac{1}{\delta}}{\lambda^2 t_1},\ a_i = \frac{1000 G^2\log\frac{1}{\delta_i}}{\lambda^2 t_i}\text{, and } \Lambda_i = 2a_{i-1} \, .
\]
Now, for each $i\in\N$, we invoke~\autoref{lem:sgd concentration details} with $A_0=a_{i-1}$, $A_1=a_i$, $T_0=t_{i-1}$, $T_1=t_i$, and $\delta'=\delta_i$.
Let us verify the two conditions. First, we verify the pull out condition as follows.
\begin{align*}
a_{i-1} + \Delta_i
&=a_{i-1} + \frac{G^2t_i\log\frac{1}{\delta_i}}{\lambda^2t_{i-1}^2} \left(\sqrt{\frac{70t_{i-1}\Lambda_i\lambda^2}{G^2
\log\frac{1}{\delta_i}}} + 50\right)\\
&= a_{i-1} + \frac{2\sqrt{70\cdot 2000}\cdot a_{i-1}}{1000} + \frac{200a_{i-1}}{1000} < 2a_{i-1} = \Lambda_i \, .
\end{align*}
Next, we verify the improvement condition $\prod_{t=t_{i-1}+1}^{t_i}(1-2\eta_t\lambda)(a_{i-1}+\Delta_i) < a_{i}$ as follows.
\[
 \frac{t_{i-1}(t_{i-1} - 1)}{t_i(t_i - 1)} \cdot 2a_{i-1} < \frac{2a_{i-1}}{4} \leq a_i \, .
\]
As $a_i\geq \frac{1000G^2(\log(1/\delta)+\log\log (t_{i-1}+1))}{\lambda^2t_{i}}$ for every $t_{i-1}+1\leq t\leq t_i$, by~\autoref{lem:sgd concentration details}, this implies that
\[
\Pr\left[\exists t_{i-1} + 1\leq t\leq t_i \, ,\ X_{t} > \frac{1000 G^2\left(\log\frac{1}{\delta}+\log\log (t+1)\right)}{\lambda^2 t} \, \middle|\, X_{t_{i-1}}\leq a_{i-1} \right] < \delta_i \, .
\]
Also, since $\sum_{i=1}^\infty\delta_i\leq\delta$ and $X_{t}\leq \frac{4G^2}{\lambda^2}$ for all $t\leq t_1$ due to the $G$-boundedness of $F$, by union bound we have
\[
\Pr\left[\exists  t\in\N,\ X_{t} > \frac{1000 G^2\left(\log\frac{1}{\delta}+\log\log (t+1)\right)}{\lambda^2 t} \right] < \delta \, .
\]
This completes the proof for the strong uniform convergence of SGD.
\end{proof}


==> main <==
\newcommand{\etalchar}[1]{$^{#1}$}
\begin{thebibliography}{AGKM16}

\bibitem[AGH{\etalchar{+}}13]{arora2013practical}
Sanjeev Arora, Rong Ge, Yonatan Halpern, David Mimno, Ankur Moitra, David
  Sontag, Yichen Wu, and Michael Zhu.
\newblock A practical algorithm for topic modeling with provable guarantees.
\newblock In {\em International Conference on Machine Learning}, pages
  280--288, 2013.

\bibitem[AGH{\etalchar{+}}14]{anandkumar2014tensor}
Animashree Anandkumar, Rong Ge, Daniel Hsu, Sham~M Kakade, and Matus Telgarsky.
\newblock Tensor decompositions for learning latent variable models.
\newblock {\em Journal of Machine Learning Research}, 15:2773--2832, 2014.

\bibitem[AGKM16]{arora2016computing}
Sanjeev Arora, Rong Ge, Ravi Kannan, and Ankur Moitra.
\newblock Computing a nonnegative matrix factorization---provably.
\newblock {\em SIAM Journal on Computing}, 45(4):1582--1611, 2016.

\bibitem[AGM12]{arora2012learning}
Sanjeev Arora, Rong Ge, and Ankur Moitra.
\newblock Learning topic models--going beyond svd.
\newblock In {\em 2012 IEEE 53rd Annual Symposium on Foundations of Computer
  Science}, pages 1--10. IEEE, 2012.

\bibitem[AYPS11]{abbasi2011improved}
Yasin Abbasi-Yadkori, D{\'a}vid P{\'a}l, and Csaba Szepesv{\'a}ri.
\newblock Improved algorithms for linear stochastic bandits.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  2312--2320, 2011.

\bibitem[AZL17]{AL17}
Zeyuan Allen-Zhu and Yuanzhi Li.
\newblock First efficient convergence for streaming k-pca: a global, gap-free,
  and near-optimal rate.
\newblock In {\em 2017 IEEE 58th Annual Symposium on Foundations of Computer
  Science (FOCS)}, pages 487--492. IEEE, 2017.

\bibitem[AZLS18]{allen2018convergence}
Zeyuan Allen-Zhu, Yuanzhi Li, and Zhao Song.
\newblock A convergence theory for deep learning via over-parameterization.
\newblock {\em arXiv preprint arXiv:1811.03962}, 2018.

\bibitem[AZLS19]{allen2019convergence}
Zeyuan Allen-Zhu, Yuanzhi Li, and Zhao Song.
\newblock On the convergence rate of training recurrent neural networks.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  6673--6685, 2019.

\bibitem[BBV04]{boyd2004convex}
Stephen Boyd, Stephen~P Boyd, and Lieven Vandenberghe.
\newblock {\em Convex optimization}.
\newblock Cambridge university press, 2004.

\bibitem[CL06]{Fan2006}
Fan Chung and Linyuan Lu.
\newblock Concentration inequalities and martingale inequalities: a survey.
\newblock {\em Internet Mathematics}, 3(1):79--127, 2006.

\bibitem[CLSH19]{chen2019convergence}
Xiangyi Chen, Sijia Liu, Ruoyu Sun, and Mingyi Hong.
\newblock On the convergence of a class of adam-type algorithms for non-convex
  optimization.
\newblock In {\em 7th International Conference on Learning Representations,
  ICLR 2019}, 2019.

\bibitem[CW20]{CW20}
Chi-Ning Chou and Mien~Brabeeba Wang.
\newblock Ode-inspired analysis for the biological version of oja{'}s rule in
  solving streaming pca.
\newblock In {\em Proceedings of Thirty Third Conference on Learning Theory
  (COLT 2020)}, volume 125, pages 1339--1343. PMLR, 09--12 Jul 2020.

\bibitem[DHK08]{dani2008stochastic}
Varsha Dani, Thomas~P Hayes, and Sham~M Kakade.
\newblock Stochastic linear optimization under bandit feedback.
\newblock {\em 21st Annual Conference on Learning Theory}, 2008.

\bibitem[DSOR15]{DOR15}
Christopher De~Sa, Kunle Olukotun, and Christopher R{\'e}.
\newblock Global convergence of stochastic gradient descent for some non-convex
  matrix problems.
\newblock In {\em Proceedings of the 32Nd International Conference on
  International Conference on Machine Learning - Volume 37}, ICML'15, pages
  2332--2341. JMLR.org, 2015.

\bibitem[DZPS18]{du2018gradient}
Simon~S Du, Xiyu Zhai, Barnabas Poczos, and Aarti Singh.
\newblock Gradient descent provably optimizes over-parameterized neural
  networks.
\newblock {\em arXiv preprint arXiv:1810.02054}, 2018.

\bibitem[Fre75]{freedman1975tail}
David~A Freedman.
\newblock On tail probabilities for martingales.
\newblock {\em the Annals of Probability}, pages 100--118, 1975.

\bibitem[GHJY15]{ge2015escaping}
Rong Ge, Furong Huang, Chi Jin, and Yang Yuan.
\newblock Escaping from saddle points—online stochastic gradient for tensor
  decomposition.
\newblock In {\em Conference on Learning Theory}, pages 797--842, 2015.

\bibitem[Har14]{hardt2014understanding}
Moritz Hardt.
\newblock Understanding alternating minimization for matrix completion.
\newblock In {\em 2014 IEEE 55th Annual Symposium on Foundations of Computer
  Science}, pages 651--660. IEEE, 2014.

\bibitem[Haz19]{hazan2019introduction}
Elad Hazan.
\newblock Introduction to online convex optimization.
\newblock {\em arXiv preprint arXiv:1909.05207}, 2019.

\bibitem[HK14]{hazan2014beyond}
Elad Hazan and Satyen Kale.
\newblock Beyond the regret minimization barrier: optimal algorithms for
  stochastic strongly-convex optimization.
\newblock {\em The Journal of Machine Learning Research}, 15(1):2489--2512,
  2014.

\bibitem[HLPR19]{harvey2019tight}
Nicholas~JA Harvey, Christopher Liaw, Yaniv Plan, and Sikander Randhawa.
\newblock Tight analyses for non-smooth stochastic gradient descent.
\newblock In {\em Conference on Learning Theory}, pages 1579--1613. PMLR, 2019.

\bibitem[HTF09]{hastie2009elements}
Trevor Hastie, Robert Tibshirani, and Jerome Friedman.
\newblock {\em The elements of statistical learning: data mining, inference,
  and prediction}.
\newblock Springer Science \& Business Media, 2009.

\bibitem[JAZBJ18]{jin2018q}
Chi Jin, Zeyuan Allen-Zhu, Sebastien Bubeck, and Michael~I Jordan.
\newblock Is q-learning provably efficient?
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  4863--4873, 2018.

\bibitem[JBNW17]{jun2017scalable}
Kwang-Sung Jun, Aniruddha Bhargava, Robert Nowak, and Rebecca Willett.
\newblock Scalable generalized linear bandits: Online computation and hashing.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  99--109, 2017.

\bibitem[JGH18]{jacot2018neural}
Arthur Jacot, Franck Gabriel, and Cl{\'e}ment Hongler.
\newblock Neural tangent kernel: Convergence and generalization in neural
  networks.
\newblock In {\em Advances in neural information processing systems}, pages
  8571--8580, 2018.

\bibitem[JNN19]{jain2019making}
Prateek Jain, Dheeraj Nagaraj, and Praneeth Netrapalli.
\newblock Making the last iterate of sgd information theoretically optimal.
\newblock In {\em Conference on Learning Theory}, pages 1752--1755. PMLR, 2019.

\bibitem[JNS13]{jain2013low}
Prateek Jain, Praneeth Netrapalli, and Sujay Sanghavi.
\newblock Low-rank matrix completion using alternating minimization.
\newblock In {\em Proceedings of the forty-fifth annual ACM symposium on Theory
  of computing}, pages 665--674, 2013.

\bibitem[JYWJ19]{jin2019provably}
Chi Jin, Zhuoran Yang, Zhaoran Wang, and Michael~I Jordan.
\newblock Provably efficient reinforcement learning with linear function
  approximation.
\newblock {\em arXiv preprint arXiv:1907.05388}, 2019.

\bibitem[KPM15]{korda2015fast}
Nathaniel Korda, LA~Prashanth, and R{\'e}mi Munos.
\newblock Fast gradient descent for drifting least squares regression, with
  application to bandits.
\newblock In {\em Twenty-Ninth AAAI Conference on Artificial Intelligence},
  2015.

\bibitem[KPR{\etalchar{+}}17]{kirkpatrick2017overcoming}
James Kirkpatrick, Razvan Pascanu, Neil Rabinowitz, Joel Veness, Guillaume
  Desjardins, Andrei~A Rusu, Kieran Milan, John Quan, Tiago Ramalho, Agnieszka
  Grabska-Barwinska, et~al.
\newblock Overcoming catastrophic forgetting in neural networks.
\newblock {\em Proceedings of the national academy of sciences},
  114(13):3521--3526, 2017.

\bibitem[KY97]{Kushner_1997}
Harold~J. Kushner and G.~George Yin.
\newblock {\em Stochastic Approximation Algorithms and Applications}.
\newblock Springer New York, 1997.

\bibitem[LG16]{L16}
Jean-Fran{\c{c}}ois Le~Gall.
\newblock {\em Brownian motion, martingales, and stochastic calculus}, volume
  274.
\newblock Springer, 2016.

\bibitem[LS99]{lee1999learning}
Daniel~D Lee and H~Sebastian Seung.
\newblock Learning the parts of objects by non-negative matrix factorization.
\newblock {\em Nature}, 401(6755):788--791, 1999.

\bibitem[Moi18]{moitra2018algorithmic}
Ankur Moitra.
\newblock {\em Algorithmic aspects of machine learning}.
\newblock Cambridge University Press, 2018.

\bibitem[Oja82]{Oja82}
Erkki Oja.
\newblock Simplified neuron model as a principal component analyzer.
\newblock {\em Journal of mathematical biology}, 15(3):267--273, 1982.

\bibitem[PKP{\etalchar{+}}19]{parisi2019continual}
German~I Parisi, Ronald Kemker, Jose~L Part, Christopher Kanan, and Stefan
  Wermter.
\newblock Continual lifelong learning with neural networks: A review.
\newblock {\em Neural Networks}, 113:54--71, 2019.

\bibitem[QDC19]{qiao2019rates}
Xingye Qiao, Jiexin Duan, and Guang Cheng.
\newblock Rates of convergence for large-scale nearest neighbor classification.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  10768--10779, 2019.

\bibitem[RR19]{richards2019optimal}
Dominic Richards and Patrick Rebeschini.
\newblock Optimal statistical rates for decentralised non-parametric regression
  with linear speed-up.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  1214--1225, 2019.

\bibitem[RSS12]{rakhlin2012making}
Alexander Rakhlin, Ohad Shamir, and Karthik Sridharan.
\newblock Making gradient descent optimal for strongly convex stochastic
  optimization.
\newblock In {\em Proceedings of the 29th International Coference on
  International Conference on Machine Learning}, pages 1571--1578, 2012.

\bibitem[SB18]{sutton2018reinforcement}
Richard~S Sutton and Andrew~G Barto.
\newblock {\em Reinforcement learning: An introduction}.
\newblock MIT press, 2018.

\bibitem[Set09]{settles2009active}
Burr Settles.
\newblock Active learning literature survey.
\newblock Technical report, University of Wisconsin-Madison Department of
  Computer Sciences, 2009.

\bibitem[Sha16]{Shamir16}
Ohad Shamir.
\newblock Convergence of stochastic gradient descent for pca.
\newblock In {\em International Conference on Machine Learning}, pages
  257--265, 2016.

\bibitem[SSBD14]{shalev2014understanding}
Shai Shalev-Shwartz and Shai Ben-David.
\newblock {\em Understanding machine learning: From theory to algorithms}.
\newblock Cambridge university press, 2014.

\bibitem[YWH19]{yu2019double}
Yue Yu, Jiaxiang Wu, and Longbo Huang.
\newblock Double quantization for communication-efficient distributed
  optimization.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  4440--4451, 2019.

\bibitem[ZSJ{\etalchar{+}}19]{zou2019sufficient}
Fangyu Zou, Li~Shen, Zequn Jie, Weizhong Zhang, and Wei Liu.
\newblock A sufficient condition for convergences of adam and rmsprop.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 11127--11135, 2019.

\end{thebibliography}

